Cap4Video: What Can Auxiliary Captions Do for Text-Video Retrieval?

Most existing text-video retrieval methods focus on cross-modal matching between the visual content of videos and textual query sentences. However, in real-world scenarios, online videos are often accompanied by relevant text information such as titles, tags, and even subtitles, which can be utilized to match textual queries. This insight has motivated us to propose a novel approach to text-video retrieval, where we directly generate associated captions from videos using zero-shot video captioning with knowledge from web-scale pre-trained models (e.g., CLIP and GPT-2). Given the generated captions, a natural question arises: what benefits do they bring to text-video retrieval? To answer this, we introduce Cap4Video, a new framework that leverages captions in three ways: i) Input data: video-caption pairs can augment the training data. ii) Intermediate feature interaction: we perform cross-modal feature interaction between the video and caption to produce enhanced video representations. iii) Output score: the Query-Caption matching branch can complement the original Query-Video matching branch for text-video retrieval. We conduct comprehensive ablation studies to demonstrate the effectiveness of our approach. Without any post-processing, Cap4Video achieves state-of-the-art performance on four standard text-video retrieval benchmarks: MSR-VTT (51.4%), VATEX (66.6%), MSVD (51.8%), and DiDeMo (52.0%). The code is available at https://github.com/whwu95/Cap4Video .

==> sections/01_introduction/v0.tex <==
\section{Introduction}
\label{sec:intro}


\begin{figure}[t]
\begin{center}
\includegraphics[width=0.98\columnwidth]{example-image}
\end{center}
\caption{Inter-class correlation maps of ``embeddings of class labels'' for 20 categories on Kinetics-400.
\textbf{Left:} The extracted textual vectors of class labels, \textbf{Right:} The ``embeddings'' from learned classifier. The color thresholds are adjusted for better understandability. Please zoom in for best view.}
% \vspace{-4pt}
\label{fig:intro_heatmap}
\end{figure}


%% BACKGROUND
% 1.先讲检索任务的意义，历史，HOW2100M，feature-level时期
% Video-text retrieval, which aims to return for a given textual query the most relevant videos, is a fundamental research task for multi-modal video-and-language understanding.
xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx 
Over the last few years, the current state-of-arts across a wide range of downstream tasks in NLP have been revolutionized by the emergence of large-scale pre-trained models, such as BERT~\cite{devlin2018bert}, GPT~\cite{GPT,GPT3}, ERNIE~\cite{zhang2019ernie} and T5~\cite{2020t5}.
Naturally, the vision-language pre-training~\cite{clip,ALIGN,yuan2021florence,yao2021filip} has also attracted a great deal of attention in the computer vision community. 
One of the most representative works is CLIP~\cite{CLIP}, a contrastive
image-text pre-training method trained with 400M image-text pairs, which builds an impressive bridge between visual and textual domains. 
Both large-scale pre-trained vision or language models can learn knowledge from more diverse data and improve the performance of downstream tasks.


% Motivation
Therefore, more recent research \wh{cite} has concentrated on directly expanding the pre-trained image-language models (\eg, CLIP~\cite{CLIP}) for the downstream text-video retrieval task.
They can benefit from the representation vectors of both texts and images, which are roughly pre-aligned in the semantic embedding space, as a result. Then, they can finish end-to-end training using the sparse frames sampling and the pre-trained image-text encoders.
In this way, these CLIP-based works achieve SOTA performance while significantly outperforming previous works.

These above works use videos and their corresponding human-annotated textual queries for cross-modal learning. 
These annotations, however, are limited and depend on the expertise of the annotator.
Meanwhile, the large-scale pre-trained language models in NLP also have made surprising breakthroughs and can be easily adapted to downstream language tasks, \eg, text generation, commonsense reasoning.
Intuitively, this leads to the question: \emph{Can we also involve the knowledge of language models to enhance video-text matching?}



% solution
% In this paper, 我们致力于如何使用GPT2模型生成的caption提升TVR检索能力。首先，考虑到方法的易拓展性和易用性，同时也希望保留GPT2模型原有的知识，我们希望对下游视频数据直接生成captions无需额外训练，换句话说就是zero-shot video captioning。这里我们使用最近的工作zero-cap（使用frozhen CLIP和frozen GPT2模型做zero-shot image captioning），将其拓展到视频上用于生成captions。然后，如何使用caption呢。第一种，我们之间将其和对应的视频构成额外的video-text pair引入训练，这个简单且直接的数据扩增方式就能带来直接的性能提升。第二，我们将caption视为视频内容的另一种表现形式。基于现有的video-text范式，引入caption-text分支（与现有方法互补），将现有范式变成query-(video & caption). 这种范式其实更符合真实场景，caption可以视为视频的title。基于这种新的范式，我们进行多源信息交互的探索，展示相应的结论。

In this paper, we focus on how to utilize the generative capabilities of pre-trained language models to improve current CLIP-based text-video matching paradigms.
We consider using the released pre-trained language model (\ie, GPT-2~\cite{GPT2}) to generate rich and diverse captions about video content in an unsupervised manner. 
To directly generate captions from any videos without extra training, we extend ZeroCap \cite{zerocap} to perform zero-shot video captioning with frozen CLIP and GPT-2 models. 
Then, how do we use these generated captions? 
1) The first intuitive way is to incorporate these captions and corresponding videos into additional video-text pairs during the training phase. This straightforward data augmentation strategy can bring significant performance improvements.
2) 

xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx 


xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx xxx 



% Exp Results
% We conduct extensive experiments and ablation studies 
% SOTAs on text-video retrieval datasets. 此外我们把video recognition视为video-text retrieval, which text is  the class name, 我们方法也在K400，anet, ucf, hmdb上取得了SOTA性能。

% Pre-training a task-agnostic model using large-scale general datasets and then transferring its learning feature representations to downstream tasks is a paradigm in many computer vision applications~\cite{CLIP,JFT300M}. 
% %
% While in the last decade, the convolutional-based models that are optimized on the ImageNet~\cite{deng2009imagenet} (more precisely, ILSVRC-2012) dataset with a supervised style dominated this field. Owing to the dramatically increasing computational capacity, now we can train models that have several magnitude more model parameters and FLOPs %\footnote{FLOPs is short for float-point operations and is widely used to measure model complexity.} 
% on significantly larger datasets in either supervised~\cite{ridnik2021imagenet21k,JFT300M,JFT3B}, weakly-supervised~\cite{CLIP,ALIGN} or self-supervised~\cite{goyal2021self,he2020momentum} style.
% %
% Recently, contrastive learning-based vision-language pre-training~\cite{CLIP} manifest their superior capabilities in improving down-streaming tasks performance such as classification~\cite{CLIP}, captioning~\cite{mokady2021clipcap}, image generation~\cite{DALLE,DALLEV2}, to name a few. These models are powerful for two reasons: i) the employed large-scale weakly-related datasets provide rich semantics and diverse representations of concepts; ii) the representation vectors of images and texts are roughly aligned in the semantic embedding space.

%% PROBLEM
% 后续也有工作改进双模态global的方式，1，2，3....。然而这种范式，既没考虑单模态冗余，也没探索细粒度对齐。
% X-pool和TS2都通过hard方式降低视频冗余。centerclip用聚类来降视频冗余。这些方法只考虑了冗余视频帧和全局文本语义的对齐，实际上文本也存在冗余，存在多余的单词(a, the)。
% 另外的方法，考虑细粒度token-wise对齐，没有考虑降冗余。
% However, the most common approach to using these models is fine-tuning the visual encoder on specific tasks. Although the rich semantics and diverse representations of concepts benefit the downstream tasks, the usage of the textual encoder is still left undiscovered.

% Motivation
% In this study, we aim to improve the transferability of such vision-language pre-training models for downstream classification tasks, with the help of their textual encoders. 
% Our intuitive insight is that if we only have the information about two similar classes, it can be difficult to distinguish them. However, comparing them to other dissimilar categories and calculating inter-class correlations could make this task easier. For example, though the ``driving car" and the ``driving tractor'' are similar, the similarity of the ``driving car'' to other classes (\eg, ``drinking'') can differ from the similarity of the ``driving tractor'' to other classes (\eg, ``drinking'').
% For a visual recognition framework, this projection matrix (classifier) can be non-rigorously considered as $c$ $d$-dim embeddings of the $c$ class labels, allowing us to explore the inter-class correlation between these learned ``embeddings'', as shown on the right side of Figure~\ref{fig:intro_heatmap}. 
% We employ the kinetics video recognition dataset~\cite{kay2017kinetics} and conduct the visual-only fine-tuning progress with the visual encoder released by CLIP~\cite{CLIP}. 
% Interestingly, these learned ``embeddings'' also reveal certain correlations after the training progress, despite being initialized randomly and optimized without knowing any textual information~\footnote{That is, optimized with cross-entropy loss with one-hot labels}.
% So is it possible to directly transfer textual knowledge to visual classifiers?
% We extract the embedded textual vectors of class labels using the textual encoders of CLIP~\cite{CLIP}, then calculate the correlation between them. The plots are given on the left side of \Cref{fig:intro_heatmap}. Not surprisingly, the extracted textual vectors of class labels exhibit certain similar correlations with that of the learned ``embeddings'', since part of them include the same verbs in their labels, such as \textit{eating $<$ something $>$}.

% use the inner product to compute the correlation between these $c$ embeddings and the visual feature vector. 
% More concretely, given a feature vector of dimension $d$ from the visual encoder, we multiply it with a projection matrix of $d \times c$ to compute the pre-softmax values (or logits) for the $c$ classes.  
%


% Motivation
% 我们捕捉双模态内的saliency，做soft的降冗余,然后做细粒度匹配。
% In this study, we aim to improve the transferability of such vision-language pre-training models for downstream classification tasks, with the help of their textual encoders. Our motivation comes from the semantic similarity among the ground-truth labels. To demonstrate this, we employ the kinetics video recognition dataset~\cite{kay2017kinetics} for the analysis. We extract the embedded textual vectors of class labels using the textual encoder released by CLIP~\cite{CLIP}. We then calculate the correlation between the embedded textual vectors. 
% The plot is shown on the left of \Cref{fig:intro_heatmap}. Not surprisingly, the extracted textual vectors of class labels exhibit certain inter-class correlations, since part of them include the same verbs in their labels, such as \textit{playing} \textless\textit{something}\textgreater. Meanwhile, the labels with different verbs show a negligible inter-class correlation, such as \textit{drinking} and \textit{driving}.
% %
% Next, we examine the final projection head of a vanilla visual recognition framework. We conduct the visual-only fine-tuning progress with the visual encoder that is also released by CLIP~\cite{CLIP}. The detailed configurations are provided in \Cref{ab:k400}. The projection head is a matrix of $d \times c$ to compute the pre-softmax values (or logits) from the $d$-dimensional feature vectors for the $c$ classes. Non-rigorously, we can consider the $d$-dimensional row vectors as the embeddings of the class labels, allowing us to explore the inter-class correlation between these learned ``embeddings'', as shown on the right side of Figure~\ref{fig:intro_heatmap}. 
% Interestingly, these learned ``embeddings'' also reveal certain correlations after the training progress, despite being initialized randomly and optimized without knowing any textual information~\footnote{That is, optimized with cross-entropy loss with one-hot labels}.

% SOLUTION
% Therefore, we suppose that the semantic information contained in the samples (images and videos) does correlate with inter-classes. Following this motivation, we replace the projection matrix with several variants: i) A projection matrix whose row vectors are randomly sampled (trivial correlation); ii) A projection matrix whose row vectors are orthogonal to each other (non-correlated). Then we replace the projection matrix with fixed embedded textual vectors that provide the ``proper'' correlation. In the empirical studies, we find that the textual knowledge significantly improves the transferability of pre-trained models, regarding both the classification accuracy and the convergence speed. Our main contributions are summarized as follows:
% \begin{itemize}
%     % \item We provide an empirical study on the correlations of the linear projection matrix for the feature transferring.
%     \item We build a new recognition paradigm to improve the transferability using knowledge from the textual encoder of the well-pretrained vision-language model.
%     \item We conduct extensive experiments on popular video and image datasets (\ie, Kinetics-400~\cite{kay2017kinetics}, UCF-101~\cite{ucf101}, HMDB-51~\cite{hmdb} and ImageNet~\cite{deng2009imagenet}) to demonstrate the transferability of our solution in many types of transfer learning, \ie, image/video recognition, zero-shot recognition, few-shot recognition. 
%     Our approach democratizes the training on large-scale video/image datasets and achieves state-of-the-art performance on video recognition tasks, \eg, 87.3\% top-1 accuracy on Kinetics-400.

% \end{itemize}



